Incremental Concept Learning via Online Generative Memory Recall

The ability to learn more and more concepts over time from incrementally arriving data is essential for the development of a life-long learning system. However, deep neural networks often suffer from forgetting previously learned concepts when continually learning new concepts, which is known as catastrophic forgetting problem. The main reason for catastrophic forgetting is that the past concept data is not available and neural weights are changed during incrementally learning new concepts. In this paper, we propose a pseudo-rehearsal based class incremental learning approach to make neural networks capable of continually learning new concepts. We use a conditional generative adversarial network to consolidate old concepts memory and recall pseudo samples during learning new concepts and a balanced online memory recall strategy is to maximally maintain old memories. And we design a comprehensible incremental concept learning network as well as a concept contrastive loss to alleviate the magnitude of neural weights change. We evaluate the proposed approach on MNIST, Fashion-MNIST and SVHN datasets and compare with other rehearsal based approaches. The extensive experiments demonstrate the effectiveness of our approach.

==> IncrementalConceptNet - arxiv/sections/abstract.tex <==
%%%%%%%%% ABSTRACT
\begin{abstract}
The ability to learn more and more concepts over time from incrementally arriving data is essential for the development of a life-long learning system. However, deep neural networks often suffer from forgetting previously learned concepts when continually learning new concepts, which is known as catastrophic forgetting problem. 
The main reason for catastrophic forgetting is that the past concept data is not available and neural weights are changed during incrementally learning new concepts.
In this paper, we propose a pseudo-rehearsal based class incremental learning approach to make neural networks capable of continually learning new concepts. 
We use a conditional generative adversarial network to consolidate old concepts memory and recall pseudo samples during learning new concepts and a balanced online memory recall strategy is to maximally maintain old memories. 
And we design a comprehensible incremental concept learning network as well as a concept contrastive loss to alleviate the magnitude of neural weights change. 
We evaluate the proposed approach on MNIST, Fashion-MNIST and SVHN datasets and compare with other rehearsal based approaches. The extensive experiments demonstrate the effectiveness of our approach.
\end{abstract}

% online sampling的作用是为了解决其他generative models中的遗忘问题，

% 摘要中的一些名词是否需要，用其他字体，比如concept contrastive loss？
% 问题在于概念和类别是否是同一回事儿？会被人diss。concepts的范围更广一些

% 文章要强调是，class incremental的，而且是构造了新的learner，并且分析了特点;
% 其他的ACGAN方法都借鉴了LwF的方法使用了不同方式的distill loss，但是这种方法只能是尽量保留原始信息而已，用fake 数据来计算soft target，并且用来存储，本身感觉就有些不太正确。。。如果能够回忆出更加清晰的样本，那么效果一定会更好。
% 是否要说生物学方面的启发呢？大脑结构学习结构什么的？ 第一遍写先不说了。。之后再完善。



==> IncrementalConceptNet - arxiv/sections/discussion.tex <==
\section{Discussion}
%todo 讨论和分析一下，在pseudo-recall的方法中，我们方法的具体贡献是什么，是否可以拓展到其他的方法中去。
In this paper, we propose a novel approach to solve catastrophic forgetting problem in class incremental learning scenario. In order to fit for class incremental learning scenario, we design a readily comprehensible network architecture named ICLNet which only need to increase the number of concept vectors in concept memory matrix while learning new concepts. 
To alleviate the catastrophic forgetting problem caused by large neural weights change, we propose a concept contrastive loss which help to concentrate the features to their corresponding concept vectors and keep away from other concept vectors. We can interpret the concept contrastive loss with ICLNet as a kind of regularization approach. 
Unlike EWC and IMM which regularize with precomputed importance weights and distillation methods \cite{2017LwF,2018ICLwGAN} which regularize  with soft targets of samples, we regularize with remoulded neural network structure and an loss function for continual learning.
We believe that redesigning computational architecture of neural networks will be a proper way to achieve efficient continual learning in the future.
On the other hand, we propose a balanced online recall strategy to make LS-ACGAN capable of incrementally consolidating generative memory with high quality in continual learning scenario.
Because of the advantage of the two proposed methods, we outperform other pseudo-rehearsal based approaches on MNIST, Fashion-MNIST and SVHN. And our ICLNet also performs better than well known rehearsal-based approach, iCaRL, in the same rehearsal scenario.

The disadvantage of our approach, which is also the disadvantage of other pseudo-rehearsal based approaches, is that we depend on 
the capability of the generative models used as recall memory. This may hinder applying pseudo-rehearsal based continual learning approaches to large scale dataset. However, the current development of generative models is very rapid. Excellent GANs like BigGAN \cite{2018BigGAN} and S$^3$GAN \cite{2019S3GAN} have been proposed and more progress will be made in the future. Hence, it is still promising to use GANs as recall memory. 

%And in another perspective, since we separately train the ICLNet and the RecallNet, it maybe computational inefficient.

In the future, we aims to combine the ICLNet and RecallNet into an integrated model to improve computational efficiency and continual learning ability. Because the implicit and explicit memory in ICLNet should help consolidate recall memory in RecallNet.
And the information contained in RecallNet should also be used to help ICLNet continually learn new concepts.



% 我们对于持续学习的问题做了一些讨论，持续学习的主要问题在于灾难遗忘，但是可以通过设计一些结构来减轻遗忘带来的问题，如果我们能够将原来的东西都记住，那么从某个方面来说，相当于从侧面绕过了灾难遗忘的因素。而且，人类本身也会发生遗忘，所以这些是不可避免的；就算是再好的Generative Models，在记忆向后传递的过程中也会逐渐损失的。
% 缺点主要是RecallNet这里，对于比较困难的样本，仍然是比较难以学习的，因为一步就很难学习，所以持续学习recallNet就更加困难了；而且将GAN与classifier分开其实有些computational inefficient，希望之后可以合在一起学，因为两个都需要训练，而不是一个整体的情况；
% 我们的观点是，用生成式模型来进行持续学习是正确的思路，因为我们不光要学习判别能力，记忆在持续学习的过程中也有着重要的作用，想要发展更加强大的学习系统就需要有更加完整的学习功能；持续学习还设计到迁移学习和元学习方面；并且，为了达到更好的持续学习效果，必定是要对传统形式的神经网络做一些调整，比如ConceptNet这种形式，因为减小了feature variance，可以更好地尽心更持续学习；

% cifar10等更大的实验之后再做就好了。。。我们可以先说可以，然后投稿之后再做把结果保存一下。。。主要需要搞清楚最新的GAN的训练trick到底是什么。。

% discuss why our method can achieve better results, 分析和总结一下各种优势，以及缺点，以及将来我们需要做的事情。。。
% 不能缺少分析呢。。。

% ConceptNet也可以作为一种regularization的方式，相比于importance weights的方法不需要计算fisher matrix，相比于distillation的方式不需要计算； 而RecallNet online strategy, 不需要筛选也不需要存储，可以方便地构建，所以这是我的方法的优势。。。 storage efficient？还是什么的呢？？

%todo 为了客服forgetting的问题，我们提出了一种新的思路，rather than regularization and distillation loss，我们可以通过改变网络的计算形式，来增加网络对旧概念的保存能力和新概念的吸收能力，通过提出concept contrastive loss，我们减少了feature variance，减小在学习新数据的时候因为旧数据效果不好而导致的bias问题。
% ！！！！！

%todo 在最后的部分中总结一下贡献吧，对于memory replay的这一类方法中，为了缓解catastrophic forgetting提供的两种思路；一个是从特征表示角度来说的；另一个是从generative replay的角度来讲的，而且还很符合一些生物人脑启发。



% Our approach simulate the learning mechanism of human learning. 从实际的角度来减缓了灾难遗忘的问题。

% 因为现在的ConceptNet与RecallNet是相互独立的，未来我们希望研究这两部分如何交互，使用ConceptNet来促进RecallNet的学习，提高持续学习的效率与效果。

% 分析缺点，computational inefficient，因为要两部训练，并且依赖于GAN的效果，我们之后要将两部分结合起来，并且利用classifier更好地促进GAN的学习。

%\section{Conclusion}
% 基于Generative
% future work, 可以考虑持续提升generative model的能力，比如使用BigGAN或者用显式的分解方式，如infoGAN相关的后续功能，例如variational UNet等，可以考虑存储一部分数据，然后再用这些数据去生成更多的旧数据。
% 将来，除了探索更高质量的生成模型方法，还可以通过提高生成模型与判别模型之间的交互来提升结果。。。
% 要去说明一下，针对持续学习，我们应该可以从结构入手设计符合持续学习的结构，提高样本回忆的质量。
%\section{Network Structures}
%\section{Addtional Experments}
% 比如可以说明能够学习不同数量的概念，随机的概念，随后的结果都是差不多的，不存在类别之间的差异。
% 可以列举和比较一下，online 和 offline情况下，生成图像质量的对比。。。？？以及不适用balance sampling的时候的结果，会导致结果好像比较麻烦哦。。。
% 其实实验中只比较online balance和offline balance，但是下面可以列举一下
% Confusion Matrix ?? 需要吗？

% 该方法最初的一些想法，是使用concepts 作为conditional 来recall images，因为concepts或许比one hot label有更多的相对信息，所以需要fixed 他们，而且这样recallnet也就需要继承参数了。。。



==> IncrementalConceptNet - arxiv/sections/experiments.tex <==
% exp1, 补充一个ConceptsNet功能的？证明一下，它的neural plasticity比正常的更强一些？
% 补充一下可以持续做类别相差较大的class 的持续学习。。。比如MNIST和Fashion-MNIST的实验，以及更长序列的训练方式，避免遗忘更加严重了。。。
% 这里方法中GAN没有继承权重，个人认为GAN继承权重的话，会在一开始生成比较好的图像，这样的话需要重新部署两个空间的映射关系，并且可能由于GAN机制的问题，出现mode collapse甚至其他的技术问题，所以我们这里仍然使用初始化的方式。。。
% 将RecallNet与GAN分开，而不是用auxiliary classifer，也是由于训练机制的问题。。。
% EWC虽然有限制，但是其实是限制不住的。。。
% 学习速度？？学习新知识的速度？？越往后学习越快。。。

\section{Experiment}
\begin{figure*}[htbp]
	\begin{center}
		%\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
		\includegraphics[width=1.0\linewidth]{Assets/visualization2d.pdf}
	\end{center}
	\caption{The 2-D features visualization of currently learned classes during training on class incremental learning tasks. (a).Fully connected classifier trained with softmax cross entropy loss. (b). ConceptNet trained with softmax cross entropy loss. (c). ConceptNet trained with Softmax cross entropy loss and concepts contrastive loss. The black stars with labels in (b)(c) denotes the concept vectors of corresponding concepts.}
	\label{fig:2d}
\end{figure*}
In this section, we perform a variety of experiments to demonstrate the advantage of our approach. We present the implementation details in section \ref{sec4.1} . To illustrate the class incremental learning procedure, we present a feature visualization in section \ref{sec4.2} . We compare the continual learning performance with recently proposed related methods in section \ref{sec4.3} . In section \ref{sec4.4} , we perform ablation experiments to demonstrate the usefulness of key components of our approach. And show more experiments in section \ref{sec4.5} and \ref{sec4.6} .

\subsection{Implementation Details}
\label{sec4.1}
\textbf{Benchmark}: We use the \textit{average incremental accuracy} benchmark protocal suggested by~\cite{2017ICaRL} to evaluate the performance. It means, in class incremental scenarios, after each class incremental task(cit), the classifier is evaluated on the combined test set consisting of new and old class samples. We evaluate and compare on three different datasets. MNIST~\cite{1998mnist} consisting of images of handwritten digits and Fashion-MNIST~\cite{2017fashion} consisting of images of different fashion clothes are resized $32\times32$ pixels in our experiment. And SVHN~\cite{2011svhn} contains cropped digits of house numbers from real-world street images. Each of these datasets contains 10 classes. We can split each dataset into 5 class incremental tasks, each of which consists of 2 randomly picked classes. In our experiments, we directly pick classes for each task in the original label order which is $['0,1', '2, 3', '4, 5', '6, 7', '8, 9']$ for better understanding.

\textbf{Networks}: For MNIST and Fashion-MNIST, the feature extractor in ICLNet consists of 3 convolutional layers with batch normalization followed by a fully connected layer. And for SVHN, the feature extractor in ICLNet consists of 6 convolutional layers with batch normalization which is the structure provided by PyTorch\cite{2017pytorch} official examples. Since the memory consolidation is more challenging for Fashion-MNIST and SVHN which contain much more variability than MNIST, we use self-attention\cite{2018selfatten} and spectral normalization\cite{2018sn} techniques in the RecallNet. The detailed network implementations can be found in supplemental materials.

All experiemnts are implemented based on PyTorch\cite{2017pytorch} framework with Adam optimizer\cite{2014adam}, learning rate 1e-4 and batch size 64. Empirically,  we set the hyperparameter $\beta=4$ and $\eta=\sqrt{d}$ where $d$ is the dimension of concept vectors.

\begin{figure*}[t]
	%todo 这个图最好可以有一个与其他方法进行对比的结果图。。就像MeRGAN中实验的那样，这样才能更好地说明事情，不然也容易被质疑; 或许列一个real sample会更加好。
	\begin{center}
		\includegraphics[width=1.0\linewidth]{Assets/recall.pdf}
	\end{center}
	\caption{The recalled samples from our RecallNet during learning 5 class incremental tasks on datasets MNIST, Fashion-MNIST and SVHN.}
	\label{fig:recall}
\end{figure*}

\begin{figure*}[htbp]
	\centering
	\includegraphics[width=1.0\linewidth]{Assets/comp.pdf}
	\caption{The average incremental accuracy for different methods during learning 5 class incremental tasks on datasets (a).MNIST, (b).Fashion-MNIST, (c).SVHN}
	\label{fig:comp}
\end{figure*}


\subsection{Visualization}
\label{sec4.2}
In this section, a toy example on MNIST dataset is presented. We reduce the output dimension of feature extractor to 2 as well as the dimension of concept vectors. So we can directly plot the features on 2-D surface for visualization. We show the class incremental learning procedure of different concepts on 5 class incremental tasks in Figure \ref{fig:2d} . Three conditions of different classifiers and losses are compared. 

In the first row, when we use traditional fully connected layer as classifier with softmax cross entropy loss, we can see that the numerical scale of feature and intra-class variance are gradually increasing as the continual learning progresses. In the continual learning scenario, when the neural networks incrementally learn new concepts, the large changes in feature scales can lead to large network weight changes. Thereby, it increases the impact of catastrophic forgetting problems. 
When train ICLNet only with softmax cross entropy loss, it reduces the feature scale but still has large intra-class feature variance as shown in the second row. 
To further reduce the intra-class feature variance, we train ICLNet with softmax cross entropy loss and concept contrastive loss as the results shown in the third row. We can observe that the features belong to the same concept concentrate to its corresponding concept vectors and keep away from other concept vectors. This phenomenon verify the purpose of concept contrastive loss. Furthermore, it also improves the continual learning performance and we show results in the ablation study \ref{sec4.4} .

\subsection{Results and Comparisons}
\label{sec4.3}

In this section, we perform both quantitative and qualitative evaluations on our approach. We compare with DGR\cite{2017DGR} and MeRGAN~\cite{2018MRGAN}, since we all belong to pseudorehearsal-based methods~\cite{1995rehearsal} and use GAN-based models for memory recall and consolidation. 
%And we also compare with iCaRL~\cite{2017ICaRL} which is a rehearsal-based method using representative examples. 
For fair comparisons, we reimplement them using the same network structures as ours in PyTorch with reference to their official code. 

The \textbf{DGR} method is originally evaluated on domain incremental learning problems. Therefore, in order to make original DGR approach fit the class incremental learning scenario, we make some reasonable modifications. Following \cite{2017DGR}, we separately train a feedforward neural network classifier and an unconditional generative adversarial network. The replayed images are stored and labeled with the most likely category predicted by the classifier trained on the previous task. However, this way may introduce some incorrect labels for continuous training and harm the classifier in continually learning new classes.

The \textbf{MeRGAN} method proposes to use a conditional GAN to replay past data and integrates the classifier into the discriminator of cGANs. It can help to avoid potential classification errors and biased sampling towards recent categories. They use replay alignment techniques to further prevent forgetting. But we compare with the version without replay alignment.

The \textbf{AuxClassifier} method refers to the auxilliary classifier in the AC-GAN of our model which also contains the ability of classification in the class incremental learning scenario. Comparing with MeRGAN, AuxClassifier does not inherit the AC-GAN parameter from previous AC-GAN. Hence, it lacks of the implicit memory of previous learned concepts.
But we use balanced online recall strategy rather than creating an extended dataset of current task and recalled samples to train.

The \textbf{Upper Bound} refers to directly train the classifier with cross entropy loss using the data of all class incremental tasks. We regard it as the performance upper bound for continual learning.

We show the comparison results on MNIST, Fahsion-MNIST and SVHN datasets in table \ref{tab: comp} . Our results outperform other pseudorehearsal methods. For MNIST, the average precison on 5 class incremental tasks of our approach is close to upper bound. However, for the Fashion-MNIST and SVHN, there is still a big gap with upper bound.

We visualize the samples of each learned concepts recalled from the RecallNet after consolidating memory for each class incremental tasks in Figure~\ref{fig:recall}. We can see that for MNIST, the RecallNet can generate clear and diverse images even after learning the last incremental task. However, for Fashion-MNIST and SVHN, although we can recognize the generated samples, they gradually lose details and variablity.

We draw the average incremental accuracy of different methods on different datasets during learning class incremental tasks in Figure~\ref{fig:comp}. We can see that our approach performs better than other pseudo-rehearsal approaches. 




% 因为incremental learning的形式有很多种，这里我们只写我们做了的这种，以及其结果，与其他方法进行一下比较，并且不仅是结果上好一些，而且方法上也更有解释性，并且相比之下更有优势一些。。。

\begin{table}[t]
	\caption{
		The average incremental accuracy$(\%)$ comparison of different methods on datasets MNIST, Fashion-MNIST and SVHN.
	}  
	%\vspace{-6pt} % 这个可以用来缩短caption与表格之间的距离。。。
	\label{tab: comp} 
	\begin{center}
		\begin{tabular}{|c|c|c|c|}
			\hline
			Method  & MNIST & Fashion-MNIST & SVHN	
			\\\hline  \hline
			AuxClassifier & 89.59  &  49.41	& 15.32 
			\\\hline 
			DGR	 &  90.19 &  61.34	&  52.34   % test
			\\\hline  
			MeRGAN	& 96.53  &  77.34	&  64.24    % test
		%	\\\hline 
		%	iCaRL	& 97.03  &  \textbf{84.69}	 & \textbf{86.30}  
			\\\hline
			Ours  	& \textbf{98.62}	& \textbf{80.79} & \textbf{72.20}   
			\\\hline 
			Upper bound & \textbf{99.24} & \textbf{93.02}  &  \textbf{96.13}	    
			\\\hline 
		\end{tabular}
	\end{center}
	\vspace{-6pt}
\end{table}


\subsection{Ablation Study}
\label{sec4.4}
\textbf{\begin{table*}[t]
		\centering
		\caption{
			The average incremental accuracy$(\%)$ comparison of using different key components in our approach.
		}  
		%\vspace{-6pt} % 这个可以用来缩短caption与表格之间的距离。。。
		\label{tab: ablation} 
		\begin{tabular}{|c|c|c|c|c|c|}
			\hline
			\multicolumn{3}{|c|}{Variants} & \multicolumn{3}{c|}{Datasets} \\ \hline
			Net Type & Recall Strategy & Loss Function &  MNIST & Fashion-MNIST & SVHN \\ \hline \hline
			\textit{TradNet} & \textit{Balanced Online Recall } & $\mathcal{L}_{CE}$ & 96.45  &  74.98 & 66.15 \\ \hline % 
			\textit{ICLNet} & \textit{Balanced Online Recall} & $\mathcal{L}_{CE}$ & 97.24  & 78.82  &  69.62 \\ \hline % 
			\textit{ICLNet} & \textit{Balanced Online Recall} & $\mathcal{L}_{CE}+\mathcal{L}_{CC}$ &  \textbf{98.62} & \textbf{80.79} & \textbf{72.20} \\ \hline
			\textit{ICLNet} & \textit{Imbalanced Online Recall} & $\mathcal{L}_{CE}+\mathcal{L}_{CC}$ & 95.21  & 73.38 & 58.45 \\ \hline % fake
			\textit{ICLNet} & \textit{Offline Balanced Recall} & $\mathcal{L}_{CE}+\mathcal{L}_{CC}$ & 93.24  & 54.38 & 43.24 \\ \hline % fake
		\end{tabular}
\end{table*}}

We perform a series of ablation experiments to demonstrate that the key components of our approach indeed improve the performance of class incremental learning. The variants are as follows. 
(\romannumeral1). Which kind of classifier do we use, the traditional fully connected layer(\textit{TradNet}) or the ICLNet structure(\textit{ICLNet}). 
(\romannumeral2). Which kind of memory recall strategy do we use, balanced online recall (\textit{Balanced Online Recall}), imbalanced online recall (\textit{Imbalanced Online Recall}) or storing recalled samples with balanced sampling(\textit{Offline Balanced Recall}).
(\romannumeral3). Which kind of loss function do we apply, only softmax cross entropy loss($\mathcal{L}_{CE}$) or with concept contrastive loss($\mathcal{L}_{CE}+\mathcal{L}_{CC}$). 
The results in table \ref{tab: ablation} show that each of proposed component of our approach makes significant contribution to class incremental learning tasks. The ICLNet with concepts contrastive loss can reduce the feature scale and intra-class variance to help alleviate forgetting problem when recalled samples are not realistic enough.
Storing recalled sample will lose the information during continual learning of RecallNet and decrease the quality of recalled samples in the subsequent tasks. 
And without balanced sampling, online recall will fail to learn to generate samples corresponding to class labels when the number of learned concepts and new concepts are extremely imbalance. Hence, it results in failure in continual learning.
%todo 分析和描述一下各种variant的具体影响，比如imbalance等，想象分析一下。

\subsection{Learn Dissimilar Concepts}
\label{sec4.5}
We conduct a concept incremetal learning experiment across MNIST and Fashion-MNIST to show that our approach also works on continually learning dissimilar concepts from different datasets.
In this experiment, we split the whole training data of MNIST and Fashion-MNIST into four class incremental tasks which contain $['0, 1, 2, 3, 4', 'Tshirt, Trouser, Pullover, Dress, Coat',$ $'5, 6, 7, 8, 9', 'Sandal, Shirt, Sneaker, Bag, Ankle boot'$ concepts respectively. 
The average incremental accuracy of our approach have still surpass other pseudo-rehearsal based approach, DGR and MeRGAN, as shown in figure \ref{fig:acrossacc}.
We also visualize the recalled samples of each learned concepts after consolidating memory for each class incremental task in figure \ref{fig:acrossvis}. The quality incates that our approach is capable of maintain the memory of dissimilar concepts.
%todo 在这里描述一下观察。。。持续学习之后的样本怎么怎么样了。。

\begin{figure}[h]
	\begin{center}
		\includegraphics[width=1.0\linewidth]{Assets/acrossvis.pdf} 
	\end{center}
	\caption{The recall samples from RecallNet after learning four class incremental tasks across dissimilar concepts.}
	\label{fig:acrossvis}
\end{figure}

\begin{figure}[h]
	\begin{center}
		\includegraphics[width=1.0\linewidth]{Assets/acrossacc.pdf} 
	\end{center}
	\caption{The average incremental accuracy for different methods during learning 4 class incremental tasks across dissimilar concepts.}
	\label{fig:acrossacc}
\end{figure}


\subsection{Compare with Rehearsal-based Method}
\label{sec4.6}
The ICLNet can also execute class incremental learning on the rehearsal-based situation which use selected representative sample set.
We compare with the well-known rehearsal-based method iCaRL which proposes to select representative samples for old class incremental tasks and use a distillation loss to train. In our reimplementation, we set the capacity of representative set $K=2000$ and use random exemplar selection rather than exemplar selection by herding since there is no substantial difference as claimed in \cite{2018revisitICL}. And we train our ICLNet with the same selected representative sample set for fair comparison. We conduct experiments on MNIST, Fashion-MNIST and SVHN and use the same the feature extractor in ICLNet and iCaRL. As shown in figure \ref{fig:rehearsal_cmp}, the ICLNet get better performance than iCaRL.


\begin{figure}[h]
	\begin{center}
		\includegraphics[width=1.0\linewidth]{Assets/rehearsal_cmp.pdf} 
	\end{center}
	\caption{The average incremental accuracy for comparing ICLNet with iCaRL on rehearsal-based learning situation.}
	\label{fig:rehearsal_cmp}
\end{figure}


%\subsection{Extension Experiments}
% todo 这些可能由于篇幅不够就不做了。。。以后再说。。% 1.当每次任务有不同的数量的概念的准确率；  2.学习速度？ 3. 可以放到附录中去。。。
% 如果实验了的话，可以画offline balance(质量差，可以用比较一般的网络来训练？？先搞这个，没有的话就算了。)，online imbalance(混乱))及online balance的最后一个采样图。。。说明问题就行了
% 注意，这里一定要写一些分析，而不能只是罗列实验结果。。。。！！！！！！！！！！！！！！！！！！ ????
%Our approach can learn different number of concept at each incremental task. Here, we will shown that our method can effective learn different number of concepts along sequential incremental task. And the more concepts we learn, the more 
% 这张图说明一下，使用Balance Sampling的好处，在某个任务上，比如连续的两类持续学习，可以观察到randomly sample的结果会很差，但是balance batch的会好很多，不用担心类别不平衡的事情，如果是存储的方法的话，就要存很多或者要和new set一样才好，这样就不太好了。 这里有两张图，拼起来。

% todo 分两部分， 一部分是说明ConceptNet有效性[可以考虑将ConceptNet用在iCaRL上来在恒明实验有效性。]，另一部分说明balance sampling的重要性[可以用训练先学习多个类别，然后再学习一个类别之后的情况来做]
% 在不同的loss以及结构方法使用的时候，结果如何，只比较自己的方法
% Concept nets在ICaRL上可以试验一下，或许会有比他设计的distillation loss更好的结果，这样也可以说明一下当前ConceptNet的真实有效性；这一点是为了说明feature variance减小之后的有效性。
% 比较online sampling的作用？ offline与online的比较，offline存储下来与训练数据相同数量的样本，这样比较公平，而且offline性能差的主要原因是由于RecallNet使用这种有限样本的时候回变差。
% 比较一下，online balance sampling 与 offline的结果， 因为是online sampling 才提出的balance sampling， offline的时候，我们只需要存储于之前训练样本一致的样本数量就可以了。
% 除了average accuracy之外，可以考虑测量Inception Score的变化，也就是avarege inception score，来看一下生成图像的持续质量评估，说明一下我们的方法应该是更好的。之和自己比较久可以了。。。实验有点儿多啊。。。
% 与finetune，以及fixed extactor finetune的方式进行比较，有篇文章中有这个数据，也可以做一下。。。
% 用简化的方式来表示吧。

==> IncrementalConceptNet - arxiv/sections/introduction.tex <==
%%%%%%%%% BODY TEXTW
\section{Introduction}
% 先这样说吧，可以之后再加详细的说明写作
The recent development of deep learning has achieved great success in a broad range of  computer vision tasks.
% \cite{2012alexnet,2016resnet,2017faster,2018deeplab}
However, it is still far away from the purpose of artificial general intelligence(AGI). 
In the real world, artificial intelligence(AI) visual systems are usually exposed to dynamic environments where new visual concepts need to learn are emerging over time. 
% 为了使AI system 更接近与人类智能，具备lifelong learning的能力是不必可少的。
In order to make the artificial visual systems move closer towards general intelligence, it is essential to make them possess the capability of \textit{continual} or \textit{lifelong learning} which means to continually learn over time by accommodating new knowledge while retaining previously learned experience\cite{2019CLreview}. 
% 上面这句话的定义与survey第一段中描述的一样，加引用，之后需要修改一下;最好引用其他地方的内容。

In traditional learning scenario, successful deep neural networks(DNNs) are usually trained using stochastic gradient descent(SGD) optimization in batch mode where all training data are given at the same time and all classes are known in advance.
However, in continual learning scenarios, we have a neural network with the capability of recognizing some learned visual concepts and want to extend its capability of recognizing more visual concepts while giving new concept data. In practice, the most pragmatic way to achieve this goal is merging the data of learned concepts with the data of new concepts and retrain a deep neural network from scratch. 
Nevertheless, this methodology is pretty inefficient, since it requires large storage space and long retraining time. And in some cases, the previously learned concept data is never available.
If we directly train a trained neural network on new concept data, its performance of recognizing previously learned concepts  will significantly decreases. This phenomenon is known as \textit{catastrophic forgetting} or \textit{catastrophic interference} \cite{1989interference,1995cls} which refers to training a model using only new information without old information can lead to a severe performance degradation to old learned knowledge. 
Therefore, developing more flexible and intelligent methodologies to overcome catastrophic forgetting problem and achieve the continual learning goal is considerably significant and meaningful. Furthermore, gradually increasing the recognition ability of neural networks is a critical step to make learning systems closer to AGI.

From the perspective of human learning, they usually exhibit a strong ability to continually learn and accumulate knowledge throughout their lifespan. 
In particular, when they learn new knowledge, the new knowledge will not interfere with previous knowledge. Therefore, the catastrophic forgetting problem does not happen in human learning systems, which is a crucial characteristic for humans to behave intelligently. This is due to the special neurophysiological and biological mechanism of learning and memory of human brain which have been widely studied\cite{1987memory,2017neural}.
%todo 下面添加引用，在review中有;或许可以简单些一下，因为这里似乎没有必要详细去写这两个理论，目前我也描述不清楚; 而且很多方法都受到了这两种方法的启发，我们的研究是咋这个基础上，对神经网络进行改进。
Among these studies, one important study is about the stability-plasticity dilemma\cite{2013stability} which refers to the extent of a learning system to be plastic in order to integrate novel information and stable in order not to severely interfere with consolidated knowledge. The lifelong learning in human brain is mediated by a rich set of neurophysiological principles that regulate the stability-plasticity balance of the different brain areas. 
Another important study is the complementary learning systems(CLS)\cite{1995cls} theory which illustrates the significant contribution of dual memory systems involving the hippocampus and the neocortex in learning and memory. It suggests that there are specialized mechanisms in the human cognitive system for protecting consolidated knowledge. The hippocampal system rapidly encodes recent experiences and exhibits short-term adapation. The long-term learning happens in neocortex systems through the activation synchronized with multiple replays of the encoded experience.
These studies of learning and memory of human brain have motivated many previous continual learning approaches\cite{2017DGR,2017DGDM,2018ICLwGAN}.
Because of the essential difference of learning mechanisms between biological neural networks and artificial neural networks, it is difficult to design one-to-one corresponding counterparts of hippocampal system and a neocortex system in artificial neural network learning systems. However, the fact that plasticity-stability balance and memory retrieval mechanism is indispensable ingredient in human learning, is convinced. 
%Therefore, in order to build an artificial continual learning system based DNNs, we should explore and utilize the memory property of DNNs.

According to different forms of deep neural networks, we can categorize the memory in artificial neural networks into three different types: implicit memory, explicit memory and recall memory.
%todo 隐性记忆是指一个训练好的神经网络的权重，它蕴含在网络的功能中;其实也和计算结构有关系，在计算结构固定的情况下。
The implicit memory refers to the learned neural weights of DNNs. Although a single connection weight may not show any concrete meanings, the whole learned neural weights in a neural network can exhibit the functionality for solving a specific task. The implicit memory is embedded in the neural weights and represents a latent form of learned knowledge.
%%这里我们认为RNN中的hidden memory也属于implicit memory，因为他们仍然是针对一个序列的所谓记忆，而不是样本间的，它的记忆功能体现在运算结构和权重之中。
The explicit memory refers to the external memory augmented in deep neural networks\cite{2014ntm,2015end,2018RNNAMU}. Compared with the implicit memory, the explicit memory is usually formed in definite structure such as a module of sequential vectors or matrix. This kind of memory can explicitly write and read to store and access information.
% 生成式记忆，是指可以明确记忆的原始知识，可以使存储原始的样本，也可以使用生成式模型来记忆原始的数据分布; 生成式记忆是一种功能记忆，表现为可以产生出原始的
The recall memory refers to the concrete memory information of previous learned knowledge. This kind of memory can be represented by generative models\cite{2013vae,2014gan} which can recall pseudo learned information.

% todo 我们现在这里没有说conceptNet的reason，直接描述方法是如何做，在method中再去叙述。
% 利用memory的方式，继承权重 implicit memory， 
% 解决balance和利用memory 的角度来提出我们的方法
% 为了解决第一个问题，我们分析了。。
% 为了达到第二个目的
% todo 下面这些写得不是很顺畅，最好换一种形式来叙述，
% 核心观点应该是分析DNN中的记忆形式，并且利用他们使DNN的model可以进行有效的持续学习。
%todo 这里要不要说CLS的启发呢？ 虽然也是和CLS启发的论文差不多。。。
In order to make deep neural networks capable of continually learning to recognize more visual concepts, we should consider both the plasticity-stability balance during learning new concepts and how to utilize different types of memory to alleviate catastrophic forgetting problem in neural network models. 
Therefore, in this paper, we propose an incremental concept learning framework based on the characteristic of different types of artificial neural networks memory. It consists of two main components: an incremental concept learning network(ICLNet) and an incremental generative memory recall network(RecallNet).

% todo 这里最好把implicit memory， explicit memory到底是什么说清楚一下好一些。。。
The ICLNet is a remoulded feedforward neural network. It consists of a trainable feature extractorand a concept memory matrix which can be regared as implicit memory and explicit memory respectively. During incremental concept learning, we gradually increase new concept vectors in the concept memory matrix to make a neural network capable of recognize new concepts. 
Traditionally, the classifier of deep neural networks is usually a fully connected layer with softmax activation function and trained with cross entropy loss. However, training in this way will lead to large feature variance\cite{2018CosineNorm,2016centerloss}, which will result in larger weights variation and harm the implicit memory during continual learning.
Hence, we propose a contrastive concept loss for ICLNet which forces the learned features into a compact representation form. In this way, the learning capability of a neural network is not limited and the ability of preserving old concepts is improved. Hence, the plasticity and stability dilemma is balanced in when continually training neural networks.

The RecallNet aims to continually retrieve old concept memories while learning new concepts and incrementally consolidate new concept memories as well as old concepts.
We train conditional generative adversarial networks(cGANs) with least square loss as the RecallNet which is regarded as recall memory. By using cGANs, we can directly recall pseudo samples of old concepts. 
While training cGANs in incremental concept learning scenarios, we will also confront forgetting problems since existing generative models are still not satisfactory.
In order to maximally maintain old concept memories while incrementally training cGANs, we propose a balanced online recall strategy. In addition, this strategy can reduce the storage cost by not storing pseudo samples and also help other pseudo-rehearsal methods in continual learning.

We conduct a series of experiments on MNIST\cite{1998mnist}, Fashion-MNIST\cite{2017fashion} and SVHN\cite{2011svhn} datasets to illustrate the effectiveness of our proposed method. Compared with other pseudo-rehearsal\cite{2017DGR, 2018MRGAN}, we achieve the state of the art performance on the class incremental learning scenario. 


% todo 上面所写的concept incremental learning或许可以换成 class incremental learning，毕竟没必要重新说，或者在后文中，提及一下，class incremental learning就是concept incremental learning
% todo 上面逻辑上有一些不完善，现在不知道怎么改了，之后再改一下，contribution 似乎没有说清楚。
% contribution有三个，按照CLS和PS-dilemma构建了学习框架， 在学习框架中，利用memory和以前DNN在持续学习中的缺点，将DNNs分成了特征提取器和Memory Pool matrix，并且提出了CCloss来减小特征方差从而避免遗忘；对于生成cGANs，为了减小他们之间的遗忘，提出了Online Sampling strategy以及concept projection的方法，让学习更好一些；

% 最后，最好讨论一下，为什么不用auxillary classifier作为分类器，因为Discriminator为了更好的生成效果，需要Lisp西祠限制，会限制学习能力。
% 还有其他能够想到的讨论问题吗？

% ------------------------------

% 然后在总体叙述一下，RecallNet和ConceptNet分别怎么干的。。。一个回忆巩固以及一个学习
% 最好说一下，ConceptNets在学习新类别的时候，继承了之前的权重，这个代表一部分memory了。然后其他的XX
% 并且在人类学习新知识的过程中，没有展示出非常严重的forgetting problem， 所以，人类的学习机制对于机器的持续学习是一个非常好的模仿对象。

%todo 这里应该用plasitic dilemma和 SGD在data distribution不平衡的情况下，导致了功能的偏移，从而遗忘以前的东西，但是不知道如何描述，先这样写，之后看到相关再改。。。
 

% 下面写，引出我们方法的原因，一个生物启发，3个memory类型的比较，一个是发现traditional classifier的缺点。。我们只能尽可能减轻遗忘。。。很难解决它。。
% 我们暂时在introduction中先不说其他方法如何，先说我们自己的就好了，在related works中叙述相关工作。
% 从
% 在这里写，很多文章都研究了lifelong learning manner， 对于plasticity的是regularization那一套。。我们提出了自己的方法。。增加外存记忆，约束特征，学习新内容时候，减少对于weights的改变，
% 从CLS理论引出使用generative replay，我们的贡献在于generative replay是online balance的，并且利用了memory。 Technically。。。XXX

% 上面这部分写biological views，一方面是stability-plasticity dilemma, 这个启发我们通过feature variance，减少权重改变；另一个是 complementary learning systems的启发，让我们能够有回忆的记忆。

% 人类具有持续学习的能力，我们从人类的学习中获得启发。很多研究发现，学习与记忆之间是相互互补的，但是由于人脑的记忆机制至今只有理论假说，并没有明确详细的运作机制，而且又由于人工神经网络与大脑神经网络的本质不同，我们只能从中得到启发，来想办法减缓遗忘，但是memory是我们可以利用的最重要因素。
% 许多文章受到这套理论的启发来构造算法，但是由于机制的不同，我们不能做一一对应的类比，但是我们必须重视记忆在持续学习中的重要性。于是我们需要重新思考人工神经网络的中记忆形式。
% episodic memory 也是一种memory。。。如果有必要的话，我们可以将它加进来，做实验进行比较。
% 我们目前可以认为，人工神经网络中有三种记忆的形式，1.隐性记忆，指网络权重，它包含和表示了最之前功能的权重； 2.显性记忆，指外存以及，可以学习读取的那种，与网络权重相匹配的记忆； 3.生成式记忆，用于产生出具体的old memory。
% 我们利用这三种记忆形式，来实现持续学习。







% ----------------

% 当我们想让我们持续学习的时候，我们必定要改变网络的结构，我们通过增加概念向量的方式来增量式地增加网络能够识别的类别；由于人工神经网络的网络功能镶嵌在各种权重的连接中，我们随意改变权重都会改变网络的功能，而且ANN使用SGD进行目标优化，当没有旧数据分布的时候，会使网络功能在优化之后完全倾向于新的数据分布，所以根据这个特点，我为了达到持续学习的目的，在人工神经网络中引入了记忆。通过记忆的回忆来补充旧数据，并且通过减小网络的特征方差来减小网络中权重的改变。

% 严格地说基于人工神经网络的学习系统与人类大脑学习系统在本质上是不同的。我们根据人工神经网络的学习与训练特点，对学习系统中的神经网络进行了改进，提出了ConceptRecallNet的方法。主要贡献在于。。。
% 通过iterative train the neural network, 在学习的过程中不断巩固旧知识，同时学习新知识。
% 构造一个记忆网络来模仿hippocampus来作为consolidate knowledge来帮助网络实现持续学习。
% 人工神经网络与人脑有本质区别，我们模仿人类能够记忆的机制，提出我们的方法实现持续的概念学习。。
% inspired by CLS and 与人工神经网络属性，我们提出了一种方法来解决持续学习的问题。
% 简单概述一下，原因以及方法描述
% 然后说一下方法的优点与贡献。。。
 
% 当我们需要增加当前网络功能的时候，需要在重新标记的数据上进行训练。我们希望人工视觉系统也能像人一样持续学习，研究这个能力是非常有意义的，比如持续系统等等，减少训练时间什么的，如果拥有持续学习的系统，或许还可以减少新样本的需求以及快速学习新的内容。

% 受到CLS theory的其他，因为记忆很重要，但是又不是单纯的模仿，因为神经机制与人工神经网络还是有很大不同的，我们探索讨论了神经网络的特性之后，提出了一种基于回忆的方法。
% 我们从memory recall的方面提出了一个新的方法，并且讨论和发现了该方法的一些缺陷，因为不论是recallnet还是concept net都是有问题的，为了更好的利用这些方法完成持续学习的任务，我们对其进行了重新设计，比如ACGAN的balance sampling和concept network的结构，以及新加入的目标函数。
% 最后我们在几个数据集上测试了一下，发现效果还不错，同类别的方法要好一些，具有一些优点，但是也有缺点。
% 贡献在于要带来新的思考，我们应该针对持续学习设计专门的神经网络结构，让持续学习更容易进行，而且并没有改变太多原来的东西；真实有效的地方在与replay的信息，以及structure所起的作用。

% 其实核心贡献是ConceptNet减小了feature variance，这也是我们的出发点，利用不完整的记忆，与能够减少遗忘的网络结构可以让持续学习更加有效。

% todo % 为了客服forgetting的问题，我们提出了一种新的思路，rather than regularization and distillation loss，我们可以通过改变网络的计算形式，来增加网络对旧概念的保存能力和新概念的吸收能力，通过提出concept contrastive loss，我们减少了feature variance，减小在学习新数据的时候因为旧数据效果不好而导致的bias问题。

% 这部分主要写，1.为什么要持续学习，重要性何在？ 2.方法理由是什么，受到什么方面的其他 3.方法是什么，简述理由和好处是什么 4.总结一下贡献。

% 但是现在神经网络虽然可以完成很好的视觉人物，但是由于神经网络训练的方法以及结构的方面的设计，导致不能够持续学习，会有灾难遗忘，遗忘的导致主要是又有神经网络牵一发而动全身。
%However, in continual learning scenarios, these deep learning models are usually suffered from the notorious \textit{catastrophic forgetting} or \textit{catastrophic interference} \cite{1989interference,1995cls} phenomenon. 
% 这里应该可以写得更清楚，更多一些解释吧。

% 当我们有一个具有一些类别分类能力的神经网络并且想要扩展它具有更多类别的识别能力的时候，如果我们直接在新的数据上训练，就会导致旧的概念的遗忘，这个现象我们成为灾难遗忘。我们可以通过存储旧数据与新数据融合在一起，来从头训练神经网络来避免灾难遗忘问题，但是这种方法inefficient并且占据存储。在一些机器学习的场景下，我们具有一定能力的模型，而没有训练它的数据，如果我们想要增加它识别新概念的能力，就需要构造更加灵活的策略。而且逐渐增加神经网络的分类功能是让学习系统更接近人工智能的必要条件，并且是非常有意义的。
% 持续学习主要是解决，存储量大，重新训练比较慢的问题。
% 也许应该加一些分析catastrophic forgetting 问题的分析？比如神经网络权重overlap等？所以加入以及系统是必要的。implicit memory interleave, 以及backpropagation 导致优化倾向。。。https://en.wikipedia.org/wiki/Catastrophic_interference

% 说一下导致灾难遗忘的原因，比如是由于implicit memory in weights 以及使用 sdg训练容易倾向于新的数据域（这个在方法部分说了吗？）
% gradient-based, backprop-trained \cite{2013compete}
% unfortunately, the network learns to adjust its parameters to generate imags of the new domain via gradient descent, and drift away from solving previous tasks.
% 在这一部分说一下，灾难遗忘的原因简单分析一下，因为优化导致倾向改变；说一下关于旧知识蕴含爱网络的权重中或者旧的数据中，一类方法在权重进行搜索，找到能够对旧任务有效又对新任务有效，然后说一下，另一类就需要原始数据进行保存数据了，真数据或者伪数据都是可以使用的；以及说明一下finetune 什么或许会影响效果，限制学习能力。。
%todo 下面这段话和上面的说法有一些重复了。。。！！！！！！！！！！！！！！
%However, this learning scheme assumes that all annotated samples are available during the training phase and, therefore, requires the retraining of the network parameters on the entire dataset in order to adapt to changes in the data distribution. 

% 在实际的问题中也是很有意义的，对于一个更加智能系统来说，我们不希望重新训练，
% 从人类的学习方式中，我们通常能够获得构造智能系统的灵感；我们根据神经网络的特性并且收到互补学习系统的启发提出了我们的方法。
% CLS 只是一部分，人类的记忆学习的内部机制有很多，我们结合当前人工神经网络的特点，来构建符合人工神经网络特性的互补记忆系统； concept matrix作为一种外部可变的记忆？并不是存储下来的，而是gradient 调整的？？ 其实就算用检索存储的方式也不一定好啊，毕竟关键的地方在于feature extractor的倾向性。



==> IncrementalConceptNet - arxiv/sections/methods.tex <==
\section{Method}
In this section, we describe the main components of our approach and explain how we design them. 
In Section~\ref{sec3.1} and \ref{sec3.2} , we describe the details of the incremental concept learning network(ICLNet) and the incremental generative memory recall network(RecallNet). 
In Section~\ref{sec3.3} , we describe the balance online recall strategy which helps to improve the continual learning ability in RecallNet.
At last, in Section~\ref{sec3.4} , we summarize the whole training procedure in an algorithm framework.

\subsection{Incremental Concept Learning Network}
\label{sec3.1}
From the perspective of training data in the continual learning scenarios, we have to face two major challenges:
(a). The new concept data has different distribution compared with old concept data. 
(b). And intact old concept data is usually not available while learning new concepts.
And from the perspective of training algorithm, we usually use stochastic gradient descent(SGD) algorithms\cite{2016sgdoverview} to update neural weights, which aims at adjusting the functionality of neural networks on current training data. And these two aspects are the main reasons for catastrophic forgetting problem happening in continually training deep neural networks. 
In order to balance the plasticity and stability in deep neural networks to allivate the catastrophic forgetting problem, we reinterpret the DNNs and utilize the implicit and explicit memory in DNNs.

The classical deep feedforward neural networks for classification tasks usually consists of a trainable feature extractor and a classifier. 
The output classifier is usually a fully connected layer which can produce raw value logits for each category. 
Followed by a softmax activation function layer, the network can predict the probabilities of each learned category for input samples. 
If the final fully connected layer classifier does not contain biases, it is equivalent to compute the inner product between input sample feature and each learnable vector in the weight matrix. 
Since the result of inner product is unbounded, if we train a classification neural network in this way, it will lead the feature extractor to produce features with large intra-class variance~\cite{2018CosineNorm,2016centerloss}, as shown in first row of figure~\ref{fig:2d}.
However, with large variance of the previous concept features, the neural networks weights become less stable during learning non-stationary data distribution in continual learning scenarios. 
The reasion is that the larger variance features make greater change in the neural weights while adapting to new concept data. Therefore, the old concept knowledge is tend to be forgotten more.
Previous methods ~\cite{2017LwF,2017ICaRL,2018ICLwGAN} use distillation loss to keep the ability of learner on previous concepts. But these methods require precomputed soft targets of replayed samples~\cite{2018ICLwGAN} or representative samples~\cite{2017ICaRL}, which increases the computational cost.

Because of previously mentioned concerns, we remould the neural network structure as ICLNet which is specifically designed for class incremental learning as shown in Figure~\ref{fig:conceptnet}.
We denote the ICLNet as $\phi^M$ with $M$ learned concepts. As illustrated in Figure \ref{fig:conceptnet}, the ICLNet consists of a trainable feature extractor $f: \chi \rightarrow \mathbb{R}^d$ and a dynamically growing concept memory matrix $\mathbb{C}$. The trainable feature extractor is an ordinary deep neural network such as multi-layer convolutional neural networks. And the neural weights of the feature extractor can be regarded as the implicit memory.
Each row vector in the concept memory matrix represents a concept prototype the network has learned. We can regard the memory matrix as the explicit memory. When the ICLNet need to learn new concepts, the concept memory matrix dynamically increase corresponding number of concept vectors. Unlike the external memory in NTM\cite{2014ntm} which learns differentiable controller to read and write memory, we directly update the concept memory matrix via gradients.

In our approach, we compute the distance $d_{ij}$ between sample features and each vector in concept memory matrix to predict the concept of samples. The closer the distance between features and concept vectors, the higher probability they belong to the corresponding concept. Specifically, we use Euclidean distance to measure the similarity. The probability of a sample $x_i$ belongs to concept $j$ is computed via a softmax function $\sigma$:
\begin{equation}
	p_{ij} = \frac{e^{-d_{ij}}} { \sum\limits_j e^{-d_{ij}}}
\end{equation}
where $d_{ij}=||f(x_i) - c_j||_2^2, j \in \{1,...,M\}, i \in \{1,...,N\}$ and $M$ is the number learned concepts of ICLNet and $N$ is the number of training samples. And we use cross entropy loss as our objective function:

\begin{equation}
\mathcal{L}_{CE} = - \frac{1}{N} \sum\limits^N_i \sum\limits^M_j y_{ij}log(p_{ij})
\end{equation}
where $y_{ij} \in \{0, 1\}$ is the groundtruth of sample $x_i$.

In the class incremental learning scenario, we need to train ICLNet with replayed samples combined with new concept data. However, directly train the ICLNet with $\mathcal{L}_{CE}$ on merged data will still lead to large intra-class feature variance in some learned concepts as shown in the second row of Figure~\ref{fig:2d}. 

In order to reduce the intra-class feature variance of learned concepts, we propose a concept contrastive loss to learn to represent the concept feature into a more compact form.
The concept contrastive loss aims at constraining the sample features to stay closer to corresponding concept vector but keep away from other concept vectors. The loss function is be formulated as following:
\begin{gather}
\mathcal{L}_{CC} =\frac{1}{N} \sum\limits^N_i \sum\limits^M_j y_{ij}*max(0, d_{ij}-\eta) \notag \\ 
+ (1-y_{ij})*min(0, d_{ij}-\beta*\eta)
\end{gather}
where $\eta$ is margin and $\beta$ is hyperparameter. 

Training the ICLNet with $\mathcal{L}_{CE}+\mathcal{L}_{CC}$ will make learned sample features near the corresponding concept vectors.
% todo 下面这一句好好写一下，学习过程中到底会发生什么事情。怎么就让遗忘减小了,权重变化小，调整new concept vectors，去适应;要不要车implict 和 explicit memory的事情呢？？
Hence, during incrementally learning new concepts in ICLNet, the learned old concept vectors in concept memory matrix are almost fixed while learning new concepts.
The neural weights of feature extractor are adjusted with smaller extent to keep old knowledge and learn new concepts.

% ！！！ 这段分析很重要，之后也可用；
% 当学习新的类别的时候，feature extractor需要将这一个类别的特征表示到一个新的区分可判别的空间位置上去，同时需要微微调整已有的类别信息；如果新类别的初始表示方差太大，在学习新类别的时候，不免需要更多的调整，这样的话，对于神经网络中的权重改变也会是巨大的，所以对导致对旧信息更大的遗忘；所以我们在特征空间尽心给分析
% 新的任务数据分布不同，而生成式模型产生的数据分布会与原来的有一些差别，我们尽可能减小这种差别。。。 但是这里说的不太合理啊。。。
% 想说的是，当在适应新的数据的时候，如果特征variance比较大的话，学习的时候参数改变也会比较大，这样就更容易较大程度低改变参数了，于是遗忘更加严重了，之前的方法中利用了distillation loss来保持能力，于是我们希望能够学习到一些比较小的特征方差来使遗忘较小得发生。
% 下面这句话缺少证据，需要找一下有没有文章中提到过这句话的，没有的话也得找一下引用，偏理论一些的，或者直接引用deep learning book
% 分散形式的用英文怎么说？
%However, in practice, training neural network in this way usually can not reach a global optimal point. Ceaselessly training the neural network will continuously scale up the weights while maintaining the generalization ability on validation set. The resulting features will also be scaled up and in divergence structure as mentioned in ~\cite{2016centerloss}. Therefore, it will bring in some negative impact on class incremental learning if we directly use such a scaled network.
% 从distillaition的角度来说一下嘛？？？似乎也不必要。。。
% 方法的具体描述，需要参考一下Matching Networks中是怎么定义的，以及语言的顺序，自己这里组织得不太好； 这里N-M的定义不太好，换掉，会和之后的冲突，或者换掉后面的；最好是这里其实不需要指定，直接用expectation
% softmax cross entropy loss
% 这一段很重要很关键，需要重新整理一下语言的顺序说一下================= 这一点没有说明白。。。还需要组织一下理由。。为什么要用contrastive concept loss呢？
% 因为在持续训练过程中，我们每次继承了上一次网络的参数，并且随机初始化了新添加的concept vectors，我们在replay和新数据上进行训练，但是由于generative model的不完美，replay的数据不可避免地有一些信息的损失，这样我们在持续训练中仍然会出现对旧概念的遗忘，我们能够获得的持续学习的信息主要来源于网络的参数与replay的数据，既然replay的数据不完美我们就需要尽可能利用ConceptNet中存储的信息；然而直接使用cross entropy训练得到的特征仍然是发散的，这样会导致特征不稳定，从而更容易发生遗忘问题，因此我们提出了一个规范化的方式，在学习中我们希望网络获得特征，与对应的概念向量的距离小于一定程度，而与其他概念向量的距离大于一定程度，这样的话，在增加心得概念时候，我们会获得更好的特征分布。从而，可以让持续学习的效果更好一些。
% 因为我们不能使用真实的原始数据，而generative model生成的数据不完美，可以在一定程度上减轻，但是还不够好，于是我们需要从前一个阶段的ConceptNet上入手，之前的方法通常使用distillation loss，来尽可能保持一致性，我们这里我使用distillation loss，而是观察到特征发散对于持续学习的影响，我们希望学习到的特征能够比较好地限制在于中心概念比较近的距离内，于是就有了
% feature diffusion problem 的说话或许欠妥
% 本质上是因为，GAN生成的数据与old 真实数据之间其实是有偏离的，也就是bias【在Memory Replay GAN中讲到了】，这种bias会导致performance shift，于是我们希望能够尽量减少这种shift，于是使用了Contrastive Concept Loss， 减小这种由于Replay data导致的shift。

% 关于distillation loss的分析，之前最好加一段描写，不然这里说明起来会感觉没有说服力--- 这一段必须重写。。。


\subsection{Incremental Generative Memory Recall Network}
\label{sec3.2}
In the concept incremental learning scenario, the intact old concept data is not available when learning new concepts. 
We propose to use a generative model to learn the distribution of old concepts as recall memory.
Currently, generative adversarial networks are the most promising generative models. In order to generate high quality samples and eliminate computational cost, we choose to use generative adversarial networks with auxiliary classifier(ACGAN) architecture which can directly generate samples for specified concepts. 
There are many candidate objective functions for training GANs, such as wasserstein generative adversarial networks(WGAN)\cite{2017wgan}, WGAN with gradient penalty(WGAN-GP)\cite{2017wgangp} and least square generative adversarial networks(LSGAN)~\cite{2017lsgan} etc.
Different from training cGANs on a single dataset, we require continually training cGANs on non-stationary datasets in continual learning scenarios. Therefore, the recall memory consolidation speed and stability are very important.
However, WGAN and WGAN-GP methods converge slowly and are hard to tune.
Therefore, we choose to use least square generative adversarial networks(LSGAN)~\cite{2017lsgan} which are more stable and faster on training ACGAN.
%todo 上面这段理由最后重新描述一下按照下面的说法
% LSGAN是更好的选择 就是说WGAN收敛速度慢，-GP计算复杂，于是我们选择简单干净与ACGAN配合更好的LSGAN。
%尽管wgan号称可以有更好的结果，但是 WGAN 需要更多计算，需要二阶梯，增加计算量，并且收敛的慢，需要更长时间的训练，我们用LSACGAN结构既能够产生出好的样本，又能够；所以在持续学习中，我们使用了LS。
%比较说明一下，其他方法也用ACGAN，但是存在问题啊；比如需要存下来再训练或者需要用classifier重新判别，这样的话会引入误差，持续学习不光是Classifier的持续学习，还涉及到RecallNet的持续学习，如果中间某一个阶段的RecallNet失败了，那么之后的学习都会fail掉。

% todo 下面GAN的描述或许可以有更好的描述吧，最好度一下
We denote the incremental generative memory recall Network(RecallNet) which can recall $M$ concepts as $\gamma_{M}$. 
When we are learning a new class incremental task(cit), we denote $\theta_{t} = (\theta_{t}^{G}, \theta_{t}^{D}, \theta_{t}^{CLS})$ as the parameter of generator, discriminator and auxillary classifier respectively within LS-ACGAN while learning the $t$th class incremental task. We alternatively train the generator and the discriminator with classifier by solving both adversarial game. The generator optimizes the following objective function: 
\begin{gather}
	\min_{\theta_t^G}  \mathcal{L}_{GAN}^{G}(\theta_t, S_t) + \mathcal{L}_{CLS}^{G}(\theta_t, S_t) \\
	\mathcal{L}_{GAN}^{G}(\theta_t, S_t) = -\mathbb{E}_{z \sim p_z, c \sim p_c }[(D_{\theta_t^D}(G_{\theta_t^G}(z, c))-1)^2] \\
	\mathcal{L}_{CLS}^{G}(\theta_t, S_t) =  -\mathbb{E}_{z \sim p_z, c \sim p_c }[y_{c} log(C_{\theta_{t}^{CLS}}(z, c)]
\end{gather}
where $S_t$ is the training set which combines recalled old concept samples and new concept samples, $p_c = \mathcal{U}\{1, M\}, p_z = \mathcal{N}(0, 1)$ are the sampling distributions.

Similarly, the discriminator and auxillary classifier optimize the following objective function:
\begin{gather}
	\min_{\theta_t^D, \theta_t^{CLS}}  \mathcal{L}_{GAN}^{D}(\theta_t, S_t) + \mathcal{L}_{CLS}^{D}(\theta_t, S_t) \\
	\mathcal{L}_{GAN}^{D}(\theta_t, S_t) = -\mathbb{E}_{(x,c) \sim S_t }[(D_{\theta_t^D}(x)-1)^2] \notag \\ 
										+ \mathbb{E}_{z \sim p_z, c \sim p_c}[D_{\theta_{t}^D}(G_{\theta_{t}^G}(z,c))^2] \\
	\mathcal{L}_{CLS}^{D}(\theta_t, S_t) =  -\mathbb{E}_{(x,c) \sim S_t }[y_{c} log(C_{\theta_{t}^{CLS}}(x))]
\end{gather}


\subsection{Balanced Online Recall}
\label{sec3.3}
% 上面其实只需要提及各部分的结构就可以了，至于如何选择，从这部分说起就好了。。。包括online Replay 和 balance sampling
% 因为RecallNet和ConceptNet都需要用到，所以列出来单独讲述，主要为了ACGAN设计的，但是训练RecallNet的时候也这么用。
% 在ICLGAN方法中，提到了bias removel由于类别不一致导致的问题，但是方法过于简单，我们需要在这里重申一下。。。
Even though LS-ACGAN can stablize training and generate decent images, there are still many limitations in the exisiting techniques. Previous approaches\cite{2017DGR,2018ICLwGAN,2018MRGAN} leverage memory replay to create an extended dataset that contains both real new concept data and recalled pseudo samples for old concept data. However, creating an extended dataset will occupy more storage space and lose information within a limited amount of stored samples. If we continually train cGANs with the extended dataset, the information of long memory will gradually lose after a long number of class incremental tasks. Because a limited amount of recalled samples of old concepts can not cover the full data distribution.
If RecallNet fails to generate satisfactory images at one class incremental task learning stage, the following class incremental tasks learning will all be influenced.

%todo 这里需要重新表达一下，中间又一次记忆损失的话，后面的都会受到影响。
% 由于以上的一些问题，我们提出了Online sampling也就是在每个batch的时候直接去sample images，这样在最大程度上保留了信息，减少了因为目前ACGAN不能够完全地吸收数据改变（因为数据量少，或者网络本身缺陷）导致的问题；并且在训练的时候，新增类别数目与旧类别的数据可能会有一些不同，那么需要保证每个batch中类别数目相同的，才能够持续学习[我们可以在附录中放一个因为类别数目不足而导致的坏结果和好结果的比较。]，我们因此提出了balance sampling的方法。这样做很有好处。
% 本质上是在每个batch中对每个类别抽取相同数量的样本，但是为了方便，我们采用随机的方法，分别从RecallNet和
Because of these mentioned problems, we propose a balanced online recall strategy. Since we usually train neural network with mini-batch stochastic gradient descent algorithm, we can directly recall old concept samples and combine with samples from new data to consist a training mini-batch. Therefore, we do not need to store the recalled old concept data.
Due to the concepts amount imbalance between the old memory and the new data, the conditional generator is not able learn to generate correct samples according to correct labels if we train RecallNet on the imbalanced image mini-batches.
And if we train ICLNet on the imbalanced batches, it also will lead to bias problems. This is confirmed by the experimental results.
Therefore, for each data batch, the amount of each concept samples should be proportional to the number of concepts in recall memory and new class incremental task.
In practice, for implementation simplicity, we proposed a balance sampling method which only requires to compute the number of samples for old concepts data and new concepts data. Assume that the training batch size is $B$ and the number of old concepts and new concepts are $M_o$ and $M_n$ respectively. We have
\begin{equation}
	B_o+B_n = B
\end{equation}
\begin{equation}
B_o/M_o = B_n/M_n
\end{equation}
where $B_o$ and $B_n$ is amount of old concept samples and new concept samples in a training batch respectively. By solving the simultaneous equations, we can get
\newcommand\round[1]{\left[#1\right]}
\begin{gather}
	B_o = \round{M_o*B/(M_o+M_n)} \notag \\
	B_n = \round{M_n*B/(M_o+M_n))}
\end{gather}
Sampling $B_o$ samples from RecallNet and $B_n$ samples from new data can consititue a class balance training batch. And we train both ICLNet and RecallNet using this strategy.


\subsection{Algorithm Framework}
\label{sec3.4}
%其实RecallNet和ConceptNet是分开的，如果我们能够获得一个非常好的RecallNet的话，那么ConceptNet也基本上可以获得一个非常好的效果了；但是本文方法中，每次RecallNet是重新initialized，注意这些细节应该写在上面地方，并且不忽略掉呢？？
% batch mix ?? 
\smallskip
\begin{algorithm}[t]
	\KwIn{New DataSet $D_{M_n}$, ICLNet $\phi_{M_o}$, RecallNet $\gamma_{M_o}$}
	\KwOut{ICLNet $\phi_{M_o+M_n}$, RecallNet $\hat{\gamma}_{M_o+M_n}$\\}
	Increase $M_n$ new concept vectors in concept memory matrix of ICLNet as $\phi_{M_o+M_n}$ \\
	\While{early stopping criterion not met}
	{
		$Tr_{batch} \leftarrow BalancedOnlineRecall(D_{M_n}, \gamma_{M_o})$ \\
		Update ICLNet $\phi_{M_o+M_n}$ by optimizing $\mathcal{L}_{CE}+\mathcal{L}_{CC}$ on $Tr_{batch}$
	}
	
	Initialize a new RecallNet $\hat{\gamma}_{M_o+M_n}$ \\
	\While{stopping criterion not met}
	{
		$Tr_{batch} \leftarrow BalancedOnlineRecall(D_{M_n}, \gamma_{M_o})$ \\
		Update RecallNet $\hat{\gamma}_{M_o+M_n}$ by optimize adversarial loss functions on $Tr_{batch}$
	}
	
	\caption{Training incremental concept learning network via incremental generative memory recall}
	\label{alg: overall}
\end{algorithm}
\smallskip
In Algorithm~\ref{alg: overall}, we present overall training procedure of our approach. When we need to learn a new class incremental task, we have a new dataset $D_{M_n}$ containing $M_n$ new concepts, the ICLNet $\phi_{M_o}$ which is capable of recognizing $M_o$ concepts and RecallNet $\gamma_{M_o}$ which can recall $M_o$ concepts samples. First, we increase $M_n$ new concept vectors in the concept memory matrix $\mathbb{C}$ of ICLNet.
Therefore, the ConceptNet $\phi_{M_o+M_n}$ can learn to distinguish $M_o+M_n$ concepts. Next, we use balanced online recall strategy to get balance training batches to train the ConceptNet. Finally, we initialize a new RecallNet $\hat{\gamma}_{M_o+M_n}$ which can learn to recall $M_o+M_n$ concepts samples. And then train the new RecallNet with balanced online recall strategy to consolidate the currently learned concepts memory.

%todo 上面其实可以说一下，vector初始化的方法的。。不过先不说了。
% todo 统一词汇，我们构造的是ConceptNet，但是用在class incremental learning上面，为了防止与之前文献冲突，说清楚就好，是class incremental tasks. concepts data
% 画一张图，或者算法框架来总体说明一下，然后再说明各个部分的设计？
% 先说哪部分？？先说那部分不要紧，可以在描述的时候指代一下就可以 。
% 在使用Memory Recall的方法中，存在着一些以往数据生成效果并不好的问题，因为生成式模型不完美，所以我们要改进分类器以及如何最大化地使用这些不完美的生成器；于是我们提出了ConceptNet和onlineSampling的方式，并且在后面实验的部分分析了这样做的好处是什么；

% 这个地方添加一下class incremental learning的定义，define，以便说明其他方法的区别；
% 然后再related works的部分， 就不要分scenario了，只说相关工作就好了。。。 
% 下面这段没必要说了
% 将concept pool作为一种外存记忆吧，differentiable的，用于与特征进行对比，这样写比较新颖一些，其实本质上是一样的。
% 相关的持续学习方法中，一般使用传统的前向神经网络作为持续学习的网络，使用softmax函数预测类别概率，在用cross entropy进行训练，但是这种方式在实际的数据上基本上不会得到收敛得结果，loss也几乎从来不为零，而且持续训练中会导致得到的参数feature不断地分散，如\cite{centerloss}文章中看到的那样，如果持续学习下去，网络的参数的scale会进一步增大。我们将这种网络用语持续学习中，在学习过程中遇到新的类别时候，通过增加最后一层的输出节点数目来判别。在这种情况下学习到的feature是发散形式的，如图所示；因此我们重新设计了一种神经网络形式，我们将神经网络作为特征提取器，最后增加一个可以学习的Concept Pool，这是一个matrix，每行代表一个concept，当有新的类别需要学习的时候，我们就增加相应类别数量的concept，用于学习。同时结合RecallNet replay的数据与新数据组成训练数据来训练。【不需要使用distillation loss，因为这个结构就有distillation的意思在里面】

% 这样做的目的是为了reduce feature variance, 因为low variance 可以减小持续学习中遗忘的影响。。。因为在持续学习中，分类器会不断地遇到新的data distribution，网络因为没有以前的数据，在适应新的data distribution的时候，就会导致网络参数对于旧数据的遗忘。。。
% 可能应该先写Memory RecallNet

%In the case of a fixed amount of neural resources, specialized mechanisms should be designed that protect consolidated knowledge from being overwritten by the learning of novel information \cite{2018CLreview}


==> IncrementalConceptNet - arxiv/sections/related_work.tex <==
\section{Related work}
In recent years, the research into continual learning is fairly compelling and has gradually gained widespread attention. 
The catastrophic forgetting effect is still a fundamental limitation for neural networks~\cite{1989interference} to continually learn new knowledge. 
It occurs when the data distribution of new tasks to learn is significantly different from previously observed data.
The main reason of the catastrophic forgetting phenomenon is that classical deep neural networks are trained with gradient-based optimization algorithms which aim at adapting neural weights in the network to fit current data distribution and loss function. 
In continual learning scenarios, the data distribution changes over time. 
When the neural network fits the new data distribution, the previously learned knowledge in the shared representational neural weights in the neural network will be overwritten by new information. Recently, many methods have been proposed for alleviating the catastrophic forgetting problem.



\subsection{Continual Learning Strategies}
% 都大概分析一下各种方法目前存在的缺陷
From the perspective of learning strategies to alleviate catastrophic forgetting problem, recent methods can be roughly divided into four categories. 

% regularization 方法包括了importance weights以及distillation 方法
\textbf{Regularization methods}.
The regularization methods alleviate catastrophic forgetting by imposing different kind of constraints while updating the neural weights\cite{2019CLreview}.  
One kind of regularization method is elastic weight consolidation(EWC) model \cite{2017EWC} and its following methods IMM \cite{2017IMM} and R-EWC \cite{2018REWC} which estimate the importance weights of a neural network for previous tasks and impose the constraint on the corresponding parameters while learning new tasks. The limitaions of this approach are that the shared parameters may contain conflicting constraints for different tasks and the importance weight matrix should be pre-estimated and stored.
Another well known regularization method is distillation. They generally use additional objective terms to regularize changes in the mapping function of a neural network. Learning without forgetting(LwF) \cite{2017LwF} enforce the predictions of a neural network for previously learned tasks to maintain similar while learning new tasks by using knowledge distillation \cite{2015distilling}. And the following work propose to use distillation on hidden activations \cite{2016less}, preserved old tasks data \cite{2017ICaRL,2018ICLwGAN} or additional dataset \cite{2019dmc} as regularization.
However, sequentially training with regularization terms usually limit the learning capability of neural networks in some extent. 

% 动态网络结构的方法，可以增加权重或者减少权重，我们的方法也是增加权重，但是增加的有限。
\textbf{Dynamic architecture methods}.
Dynamic architecture methods dynamically change the architecture of neural networks to accommodate new neural resources to learn new knowledge. The progressive networks \cite{2016progressivenn} approach proposed an architecture with explicit support for transfer learning across sequences of tasks. It expands the architecture by allocating new network branches with fixed capacity to learn new information.
Dynamically expanding network(DEN) \cite{2017DEN} can incrementally learn new tasks by increasing the number of trainable parameters. DEN is efficiently trained in an online
manner by performing selective retraining, and automatically determine how much neural networks capacity to expand. 
Fixed expansion layer(FEL) network\cite{2013ensembleCF} mitigates the forgetting by selectively update neural weights in the network rather than expanding the neural weights during continual learning.
Comparing with dynamic architecture methods, our approach only dynamically increase new concept vectors in concept memory matrix.
% todo 看一下别人怎么说这类方法的缺点，然后突出我们方法的优点。

% 分为 rehearsal 和 pseudo rehearsal 谈谈缺点和代表性方法就好了。
\textbf{Rehearsal based methods}.
The rehearsal based approaches select and store real representative samples from previous task training task which can maintain the information the past. ICaRL \cite{2017ICaRL} proposed a practical strategy for simulaneously learning a nearest-mean-of-exemplars classifier and a feature representation in the class incremental learning setting. ICaRL used \textit{herding} to create a fixed-sized represetation set of previous task data samples and the knowledge distillation to maintain past knowledge. Gradient episodic memory(GEM) \cite{2017GEM} and \cite{2018ICLwGAN} also require part of the old data. The main difference lies on how to select the representative exemplars and how to use the representative exemplars to help maintain knowledge of past tasks. The existing limitations of rehearsal based approaches is that it violates the data availability assumption and requires additional storage space. The continual learning performance will be influenced by the quality and quantity of stored representative examplars. 
Furthermore, in some real world applications, due to the privacy and legal concerns, real data may not be allowed to be stored for a long period of time\cite{2018ICLwGAN}. 


\textbf{Pseudo-rehearsal based methods}.
The pseudo-rehearsal based methods \cite{2017DGR,2017DGDM,2018MRGAN,2018ICLwGAN} take inspiration from the CLS theory and make use of different promising generative models to learn the data distribution of previous tasks. During continually learning new tasks, the old task knowledge should be complemented by memory replay from learned generative models. The deep generative replay(DGR)\cite{2017DGR}, Memory Replay GANs \cite{2018MRGAN} and \cite{2018ICLwGAN} utilize variants of generative adversarial networks(GAN)\cite{2014gan} as generative memory. The deep generative dual memory network(DGM)\cite{2017DGDM} utilizes variational autoencoder(VAE)\cite{2013vae} as the long-term memory which stores information of all previously learned tasks. Our approach belongs to pseudo-rehearsal based method. In order to maintain information of generative models during sequentially learning new tasks, we propose a balanced online recall stratey which a general strategy and can be applied to other pseudo-rehearsal approaches.



\subsection{Continual Learning Scenarios}
%todo 这个地方参考那篇文章来看一下吧，怎么写合适
Although promising results are reported by many methods, the experimental protocols and continual learning scenarios are different in their evaluation. And different continual learning scenarios have different learning difficulty levels. But they all confront catastrophic forgetting.
Therefore, from the perspective of learning scenarios, we can divide three distinct continual learning scenarios\cite{2018RTF}. 

%todo as shown in figure X
\textbf{Task incremental learning scenario}. In this scenario, a new output-layer should be appended to the neural network while learning a new task. But during inference, the task identity should be provided to select which output-layer to use.

\textbf{Domain incremental learning scenario}. In this scenario, the same output-layer is shared while learning a new task. Therefore, for different learning tasks, they are constrained to have the same number of output units. And during inference, the task identity is also required. 

\textbf{Class incremental learning scenario}. In this scenario, the model can incrementally learn to recognize new classes and do not require to provide task identity during inference. There is only one incremental output-layer which continually increase the number of output units during learning new classes. In this paper, we refer the incremental concept learning as the same meaning with class incremental learning.

\begin{figure*}[t]
	\begin{center}
		\includegraphics[width=1.0\linewidth]{Assets/ICLNetArchitecture.pdf}
	\end{center}
	\caption{The ICLNet architecture for class incremental learning tasks.}
	\label{fig:conceptnet}
\end{figure*}


% this part talk about learning scenarios, we can merge them into related works
% 由于持续学习的定义繁多，我们这里的目的是XXX
% 在这里或者introduction的最后一段说明一下，具体的持续学习scenario； 可不可以直接说沿用某个文章中的说法，简单叙述一下，将scenario 分为三类，我们主要按照第三种方式来比较。

%也许这里不许要说这么多没用的，因为我们就是提出一种方法而已，没有比较讲其他类型的方式，因为这是一篇视觉的文章，只要说明与主题方法相关的方法就好了--之后将这里删减一下，写了的目的是为了总结和梳理一下。

% this part talk about learning stratgy
% 这部分写：1.相关方法的分类 2.对于问题的定义记忆评价标准的设定。

% 因为最近的一些论文中都有比较好的相关工作的综述而且也有review，那么这一部分该怎么写更合适呢？全部说一遍，还是只说与自己最相关的几种呢？
% 我们可以在前面不说related works，只在后面讨论的时候说一下现有的解决持续学习的一些经典方法以及各种方法存在的问题，之后我们再说明一下我们的方法虽然不完美，但是在一定程度上做出来贡献，分析了目前你的一些问题。

% EWC等通过限制权重来持续学习，重点在于如何保持对以前有用的权重，但是权重之间是相互关联的，虽然说存在于之前任务更加相关的权重，但是改变之后，也会涉及到各种地方的改变，所以这种方法很困难，也是所有方法中表现最不好的。
%使用存储代表性样本的方法，如iCaRL，缺点主要是占用了更多的数据存储空间，而且要存哪些样本以及存储多少样本，都是有待研究的，更重要的是如何使用distillation loss 来通过存下来的样本更好地保持对以前任务的记忆，关键之处在于利用了真实的信息，来约束以前的样本了。
%使用生成式模型的方法，如DGR等，缺点在于目前目前生成式模型本身是有局限的，而且在训练生成式模型的时候还要训练分类器，增加了计算量，而且使用

% 使用distillation loss的目的其实是保证网络对于原始问题的输入输出关系不变，比如LwF用新数据distillation，保证了新输入在旧节点处的输入输出对应不变，而iCaRL是用少量的旧数据保证了原来的weighs不变的情况，那么是否可以结合LwF与iCaRL呢？让iCaRL不要用旧数据呢？

% 这种方式依赖生成模型的表现，如果有一个表现不好的话，之后的表现就是灾难的；
% 因此，整合优势，我们需要设计符合持续学习结构的网络以及约束，并且要利用其要将旧的记忆用其他的方式表达出来。
% todo 这里还没有说，我们方法与他们方法之间的key difference的比较，在这里说，还是在后面说呢？？如何更好地突出我的贡献？？


